Motion Primitives-based Navigation Planning using Deep Collision Prediction

This paper contributes a method to design a novel navigation planner exploiting a learning-based collision prediction network. The neural network is tasked to predict the collision cost of each action sequence in a predefined motion primitives library in the robot's velocity-steering angle space, given only the current depth image and the estimated linear and angular velocities of the robot. Furthermore, we account for the uncertainty of the robot's partial state by utilizing the Unscented Transform and the uncertainty of the neural network model by using Monte Carlo dropout. The uncertainty-aware collision cost is then combined with the goal direction given by a global planner in order to determine the best action sequence to execute in a receding horizon manner. To demonstrate the method, we develop a resilient small flying robot integrating lightweight sensing and computing resources. A set of simulation and experimental studies, including a field deployment, in both cluttered and perceptually-challenging environments is conducted to evaluate the quality of the prediction network and the performance of the proposed planner.

==> SystemOverview.tex <==
LMF inherited the collision-tolerance design of the Resilient Micro Flyer~\cite{Paolo2020RMF}. It is integrated a sensor suite including a Realsense T265 tracker which is fused with the IMU inside the autopilot to estimate the speed, orientation and angular rate of the robot; a Realsense D455 sensor to obtain the depth data and a range sensor to regulate the height of the robot. The ORACLE planner and the low-level PID controllers to control the velocity, height and yaw angle of the robot are implemented onboard a Jetson Xavier NX.

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
    \includegraphics[width=0.6\columnwidth]{EPS/LMF_front.jpg}
\caption{LMF components.}\label{fig:radmfmotivation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
